Typed Operational Semantics for Dependent Record Types

Typed operational semantics is a method developed by H. Goguen to prove meta-theoretic properties of type systems. This paper studies the metatheory of a type system with dependent record types, using the approach of typed operational semantics. In particular, the metatheoretical properties we have proved include strong normalisation, Church-Rosser and subject reduction.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{T. Hirschowitz (Ed.): Types for Proofs and Programs 2009 (TYPES 2009). \\
EPTCS 53, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.53.3}{10.4204/EPTCS.53.3}}
\pdfoutput=1

